A literature survey of the quality economics of defect-detection techniques

Over the last decades, a considerable amount of empirical knowledge about the efficiency of defect-detection techniques has been accumulated. Also a few surveys have summarised those studies with different focuses, usually for a specific type of technique. This work reviews the results of empirical studies and associates them with a model of software quality economics. This allows a better comparison of the different techniques and supports the application of the model in practice as several parameters can be approximated with typical average values. The main contributions are the provision of average values of several interesting quantities w.r.t. defect detection and the identification of areas that need further research because of the limited knowledge available.

==> costs.tex <==
\section{Software quality costs}
\label{sec:costs}

\emph{Quality costs} are the costs associated with preventing, finding,
and correcting defective work.
Based on experience from the manufacturing area
quality cost models have been developed explicitly for software, e.g.\ 
\cite{slaughter98}.
These costs are divided into \emph{conformance} and \emph{nonconformance}
costs, also called \emph{control costs} and \emph{failure of control costs}. 
The former comprises all costs that need to be spent to build the software in
a way that it conforms to its quality requirements. This can be further
broken down to \emph{prevention} and \emph{appraisal} costs. Prevention 
costs are for
example developer
training, tool costs, or quality audits, i.\,e.~costs for means to prevent
the injection of faults. The appraisal costs are caused by the usage of 
various types of tests and reviews.

The \emph{nonconformance} costs come into play when the software does not
conform to the quality requirements. These costs are divided into
\emph{internal failure} costs and \emph{external failure} costs. The
former contains costs caused by failures that occur during development,
the latter describes costs that result from failures at the client.
A graphical overview is given in Fig.~\ref{fig:costs_overview}. Because
of the distinction between prevention, appraisal, and failure costs this
is often called \emph{PAF} model.
 
\begin{figure}[h]
  \centering \includegraphics[width=8cm]{costs}
  \caption{Overview over the costs related to quality}
  \label{fig:costs_overview}
\end{figure}

We add further detail to the PAF model
by introducing the main types of concrete costs that are important for
defect-detection techniques. Note that there are
more types that could be included, for example, maintenance costs.
However, we concentrate on a more reliability-oriented view.
The appraisal costs
are detailed to the \emph{setup} and \emph{execution} costs. The former
constituting all
initial costs for buying test tools, configuring the test environment,
and so on. The latter means all the costs that are connected to actual
test executions or review meetings, mainly personnel costs.

On the nonconformance side, we have \emph{fault removal} costs that can
be attributed to the internal failure costs as well as the external
failure costs. This is because if we found a fault and want to remove it,
it would always result in costs no matter whether caused in an internal
or external failure. Actually, there does not have to be a failure at all.
Considering code inspections, faults are found and removed that have never
caused a failure during testing. It is also a good example that the removal
costs can be quite different regarding different techniques. When a test
identifies a failure, there needs to be considerable effort spent to find
the corresponding fault. During an inspection, faults are found directly.
Fault removal costs also contain the costs for necessary re-testing and
re-inspections.

External failures also cause \emph{support} costs. These are all costs
connected to customer care, especially the effort from service workers
identifying the problem. Finally, \emph{compensation} costs could be part
of the external failure costs, if the failure caused some kind of damage
at the customer site. We might also include further costs such as loss of 
sales because of bad
reputation in the external failure costs but do not consider it explicitly.

